Dimensionality Reduction and Anomaly Detection for CPPS Data using Autoencoder

Unsupervised anomaly detection (AD) is a major topic in the field of Cyber-Physical Production Systems (CPPSs). A closely related concern is dimensionality reduction (DR) which is: 1) often used as a preprocessing step in an AD solution, 2) a sort of AD, if a measure of observation conformity to the learned data manifold is provided. We argue that the two aspects can be complementary in a CPPS anomaly detection solution. In this work, we focus on the nonlinear autoencoder (AE) as a DR/AD approach. The contribution of this work is: 1) we examine the suitability of AE reconstruction error as an AD decision criterion in CPPS data. 2) we analyze its relation to a potential second-phase AD approach in the AE latent space 3) we evaluate the performance of the approach on three real-world datasets. Moreover, the approach outperforms state-of-the-art techniques, alongside a relatively simple and straightforward application.

==> AD.tex <==
\section{Anomaly detection}\label{sec:ad}



==> DR.tex <==
\section{Dimensionality reduction}\label{sec:dr}




==> synthetic.tex <==
\subsection{Synthetic data}
Our goal is to 
We use the specific scheme for generating synthetic data motivated on later described analyzed real world examples. The schema allows us to scale complexity of the problem in several directions. For each problem we will assume sufficient amount of available data. The parameters are:
\begin{itemize}
\item Dimensionality of the latent space (intrinsic dimensionality)
\item Dimensionality of the observation space
\end{itemize}

The pool of nonlinearities is the following:
\begin{enumerate}
\item $x_k = x_i x_j$ (e.g. $P~UI$)
\item $x_j = x_i ^ 3$ (e.g. $P~v^3$)
\item $x_i = x_i(t), x_j = x_j(t)$ (e.g. as a consequence of control)

\end{enumerate}
